Optimization of Information Rate Upper and Lower Bounds for Channels with Memory

We consider the problem of minimizing upper bounds and maximizing lower bounds on information rates of stationary and ergodic discrete-time channels with memory. The channels we consider can have a finite number of states, such as partial response channels, or they can have an infinite state-space, such as time-varying fading channels. We optimize recently-proposed information rate bounds for such channels, which make use of auxiliary finite-state machine channels (FSMCs). Our main contribution in this paper is to provide iterative expectation-maximization (EM) type algorithms to optimize the parameters of the auxiliary FSMC to tighten these bounds. We provide an explicit, iterative algorithm that improves the upper bound at each iteration. We also provide an effective method for iteratively optimizing the lower bound. To demonstrate the effectiveness of our algorithms, we provide several examples of partial response and fading channels, where the proposed optimization techniques significantly tighten the initial upper and lower bounds. Finally, we compare our results with an improved variation of the \emph{simplex} local optimization algorithm, called \emph{Soblex}. This comparison shows that our proposed algorithms are superior to the Soblex method, both in terms of robustness in finding the tightest bounds and in computational efficiency. Interestingly, from a channel coding/decoding perspective, optimizing the lower bound is related to increasing the achievable mismatched information rate, i.e., the information rate of a communication system where the decoder at the receiver is matched to the auxiliary channel, and not to the original channel.

==> help1.tex <==
% Comment: arXiv-version of paper



\section{Source and Channel Models}
\label{sec:channel:models:1}


CCCCC Do we need to assume that all output symbols can be produced for all
valid branches?

CCCCC Make sure that $(QW)$ is defined somewhere.

Before presenting source and channel definitions, it is useful to define the
following index set.

\begin{Definition}{The Index Set}
  \label{def:notation:indices:1}

  We assume $N$ to be a positive integer. We define the following index set
  \begin{alignat*}{2}
    \sIN
      &\defeq
         [-N+1,N]
     &&= \{ -N+1, \ldots, N \}.
  \end{alignat*}
  Observe that the size of the set is $|{\sIN}| = 2N$. Note that in our
  results, we are mainly interested in the limit $N \to \infty$
\end{Definition}


\begin{figure}
  \begin{center}
    \epsfig{file=figs/source_channel_prob_models3.fig.eps, width=0.5\linewidth}
  \end{center}
  \caption{Block diagram of the source, the original (forward) channel, the
    ``output source'', the backward channel, the the auxiliary forward
    channel, and the auxiliary backward channel under consideration.}
  \label{fig:source:channel:prob:models:1}
\end{figure}


Consider the block diagram in Fig.~\ref{fig:source:channel:prob:models:1}
which shows a source and a so-called original channel. We assume that both are
fixed and that we would like to find good upper and lower bounds on the
information rate of this source/channel pair. Our upper bounding technique
will use a so-called forward auxiliary channel whose input and output alphabet
matches the input and output alphabet, respectively, of the original channel.
The tightening of the upper bound will be achieved by optimizing the
parameters of the auxiliary channel. Similarly, our lower bounding technique
will use a so-called backward auxiliary channel whose input and output
alphabet matches the input and output alphabet, respectively, of the original
channel. The tightening of the upper bound will be achieved by optimizing the
parameters of the auxiliary channel.


\subsection{\textbf{Source Model}}
\label{sec:source:model:1}


\begin{Definition}{Source}
  \label{def:source:model:1}

  In this paper we only consider sources that are discrete-time, stationary,
  and ergodic and that produce a sequence $\ldots, X_{-1}, X_0, X_1, \ldots$,
  where $X_{\ell} \in \setX$ for all $\ell$. We assume that the alphabet
  $\setX$ is finite and that for any $i < j$ the pmf is given by
  $P_{\vX_{i}^{j}}(\vx_{i}^{j})$. In the following, we will use the
  abbreviation $Q(\vx_{i}^{j}) \defeq P_{\vX_{i}^{j}}(\vx_{i}^{j})$ for any $i
  \leq j$.
\end{Definition}



\subsection{\textbf{Finite-State Machine Channels (FSMCs)}}
\label{sec:finite:state:channel:models:1}



Many of the original channels that we will consider can be described as
FSMCs.\footnote{Note that Gallager~\cite{Gallager:68} calls them finite-state
  channels (FSCs).}


\begin{Definition}{Finite-State Machine Channels (FSMCs)}
  \label{def:finite:state:channel:models:1}

  A time-independent, discrete-time finite-state machine
  channel~\cite{Gallager:68} has an input process $\ldots, X_{-1}, X_0, X_1,
  \ldots$, an output process $\ldots, Y_{-1}, Y_0, Y_1, \ldots$, and a state
  process $\ldots, S_{-1}, S_0, S_1, \ldots$, where $X_{\ell} \in \setX$,
  $Y_{\ell} \in \setY$, and $S_{\ell} \in \setS$ for all $\ell \in {\mathbb
    Z}$. We assume that the alphabets $\setX$, $\setY$, and $\setS$ are
  finite. Let us define the following finite windows of the FSMC states,
  inputs, and outputs as:
  \begin{align}
    \vs
      &\defeq
         {\vs}_{-N+1}^{N},
    \quad\quad
    \vx
       \defeq
         \vx_{-N+1}^{N},
    \quad\quad
    \vy
       \defeq
         \vy_{-N+1}^{N}.
  \end{align}
  Unless otherwise stated, we condition all FSMC-related probabilities on an
  initial state, such as $s_{-N}$. The joint FSMC conditional pmf decomposes
  as
  \begin{align}
    P_{\vS,\vY | \vX, S_{-N}}
      (\vs, \vy | \vx, s_{-N})
      &= \prod_{\ell \in \sIN}
           P_{S_{\ell},Y_{\ell} | S_{\ell-1}, X_{\ell}}
             (s_{\ell},y_{\ell} | s_{\ell-1}, x_{\ell}) \\
      &= \left(
           \prod_{\ell \in \sIN} P_{S_{\ell} | S_{\ell-1}, X_{\ell}}
                                 (s_{\ell} | s_{\ell-1}, x_{\ell})
         \right)
         \cdot
         \left(
           \prod_{\ell \in \sIN} P_{Y_{\ell} | S_{\ell-1}, X_{\ell},S_{\ell}}
                                 (y_{\ell} |  s_{\ell-1}, x_{\ell}, s_{\ell})
         \right),
  \end{align}
  where $P_{S_{\ell} | S_{\ell-1}, X_{\ell}}$ and $P_{Y_{\ell} | S_{\ell-1},
    X_{\ell},S_{\ell}}$ are referred to as the FSMC state transition
  probability and channel law in each state transition, respectively and are
  independent of time index $\ell$. In the following, we will use the notation
  \begin{align}
    W(s_{\ell}| s_{\ell-1}, x_{\ell})
      &\defeq
         P_{S_{\ell} | S_{\ell-1}, X_{\ell}}(s_{\ell} | s_{\ell-1}, x_{\ell}), \\
    W(y_{\ell} | s_{\ell-1}, x_{\ell}, s_{\ell})
      &\defeq
         P_{Y_{\ell} | S_{\ell-1}, X_{\ell},S_{\ell}}
           (y_{\ell} |  s_{\ell-1}, x_{\ell}, s_{\ell}), \\
    W(\vs,\vy |\vx,s_{-N})
      &\defeq
         P_{\vS,\vY |\vX, S_{-N}}
           (\vs,\vy |\vx, s_{-N}).
  \end{align}

\end{Definition}


\begin{figure}
  \begin{center}
    \epsfig{file=figs/trellis_channel1_mod3.fig.eps, width=0.5\linewidth}
  \end{center}
  \caption{Trellis representation of the finite-state machine behind an
    FSMC. Because of the assumed time-invariance, the branch labels in every
    trellis section are the same. Therefore, we have shown these branch labels
    only in one trellis section.}
  \label{fig:trellis:channel:notation:1}
\end{figure}


\begin{figure}
  \begin{center}
    \epsfig{file=figs/fsc_gilbert_elliott1_mod2.fig.eps, width=0.2\linewidth}
  \end{center}
  \caption{Trellis section of the trellis representation of the finite-state
    machine behind a Gilbert-Elliott channel. State ``$1$'' corresponds to the
    bad state ``$\bad$'' and state ``$2$'' corresponds to the good state
    ``$\good$''.}
  \label{fig:trellis:section:gilbert:elliott:channel:1}
\end{figure}


\figref{fig:trellis:channel:notation:1} shows how the finite-state machine
behind a typical FSMC can be represented by a trellis. This specific FSMC has
$4$ states, namely $\setS = \{ 1, 2, 3, 4 \}$, and two input symbols, namely
$\setX = \{ -1, +1 \}$. To a branch going from state $i$ to state $j$ we
associate a label like $(x_{ij}; p_{ij})$: it shows the probability $p_{ij}$
with which this state transition is chosen in case that the channel input
symbol is $x_{ij}$.


\begin{Example}{Partial Response Channel}
  \label{ex:partial:response:channel:1}

  The trellis in \figref{fig:trellis:channel:notation:1} actually represents
  the trellis of the finite-state machine that is behind a so-called partial
  response channel. Such a channel can be described by
  \begin{align}\label{eq:fir}
    y_{\ell}
      &= \mu
         \left(
           \sum_{m=0}^{M}
             h_m x_{\ell-m}
             +
             n_{\ell}
         \right).
  \end{align}
  Here, $\mu$ is a quantization function that maps elements of $\mathbb{R}$ to
  $\setY$, and $\{ x_{\ell} \}$, $\{ y_{\ell} \}$, $\{ n_{\ell} \}$, $\{ h_m
  \}$ represent the channel input process, the channel output process, an
  additive noise process, and the filter coefficients, respectively. Assuming
  the channel input alphabet to be $\setX = \{ -1, +1 \}$ and the memory
  length to be $M = 2$, we see that in \figref{fig:trellis:channel:notation:1}
  the state $S_{\ell} = 1$ corresponds to $(X_{\ell-1},X_{\ell}) = (-1,-1)$,
  the state $S_{\ell} = 2$ corresponds to $(X_{\ell-1},X_{\ell}) = (-1,+1)$,
  the state $S_{\ell} = 3$ corresponds to $(X_{\ell-1},X_{\ell}) = (+1,-1)$,
  and the state $S_{\ell} = 4$ corresponds to $(X_{\ell-1},X_{\ell}) =
  (+1,+1)$.
\end{Example}


\begin{Example}{Gilbert-Elliott Channel}
  \label{example:gilbert:elliott:channel:1}

  The Gilbert-Elliott channel~\cite{Gallager:68} has the state alphabet
  $\set{S} = \{ \good, \bad \}$, \ie, a ``good'' state and a ``bad'' state,
  the input alphabet $\setX = \{ 0, 1 \}$, and the output alphabet $\{ 0,1
  \}$. One defines $W(s_{\ell},y_{\ell} | s_{\ell-1},x_{\ell}) \defeq
  W(s_{\ell} | s_{\ell-1}) \cdot W(y_{\ell} | s_{\ell-1},x_{\ell})$ with
  $W(\bad | \good) = \pbad$, $W(\good | \bad) = \pgood$, and $W(y_{\ell} |
  s_{\ell-1},x_{\ell})$ is a binary symmetric channel (BSC) with cross-over
  probability $\epsgood$ when $s_{\ell-1} = \good$ and a BSC with cross-over
  probability $\epsbad$ when $s_{\ell-1} = \bad$, respectively. A trellis
  section of the trellis representation of the finite-state machine behind
  such a channel is shown
  in~\figref{fig:trellis:section:gilbert:elliott:channel:1}.
\end{Example}


It is useful to introduce the FSMC branch random variable $B_{\ell} \defeq
(S_{\ell-1}, X_{\ell}, S_{\ell})$. The initial state of a branch $b_{\ell}$ at
time index $\ell$ will then be denoted by $s_{\ell-1}(b_{\ell})$, the channel
input symbol by $x(b_{\ell})$, and the final state by $s_{\ell}(b_{\ell})$. It
can easily be seen that without loss of generality we can assume that for any
triple $(s_{\ell-1}, x_{\ell}, s_{\ell})$ there is at most one branch in the
trellis that starts in state $s_{\ell-1}$, has input symbol $x_{\ell}$ and
ends in state $s_{\ell}$. In that sense, in the following we will use the
notation
\begin{align}
  W(y_{\ell} | b_{\ell})
    &\defeq
       P_{Y_{\ell} | B_{\ell}}
         (y_{\ell} |  b_{\ell})
     = P_{Y_{\ell} | S_{\ell-1}, X_{\ell},S_{\ell}}
         (y_{\ell} |  s_{\ell-1}, x_{\ell}, s_{\ell})
     = W(y_{\ell} |  s_{\ell-1}, x_{\ell}, s_{\ell})
\end{align}
for $b_{\ell} = (s_{\ell-1}, x_{\ell}, s_{\ell})$. Similarly to $\vs$, $\vx$,
and $\vy$, we also define $\vb \defeq {\vb}_{-N+1}^{N}$ which helps us to
define
\begin{align}
  W(\vb, \vy | \vx, s_{-N})
    &\defeq
       W(\vs, \vy | \vx, s_{-N}).
           \label{eq:from:state:and:symbol:seq:to:branch:seq:1}
\end{align}
In this and upcoming similar expressions, $\vx$ and $\vs$ are implicitly given
by $\vb$, \ie, $\vx = \vx(\vb)$ and $\vs = \vs(\vb)$.

In this paper, we consider only FSMCs that are indecomposable, as defined by
Gallager~\cite{Gallager:68}, \ie channels where, roughly speaking, the
influence of the initial state fades out with time for every possible channel
input sequence. Feeding such a channel with a stationary and ergodic source
results in input and output processes that are jointly stationary and ergodic.

Therefore, when feeding an indecomposable FSMC with a source as in
Def.~\ref{def:source:model:1} we will use the notation
\begin{align}
  W(\vy | \vx, s_{-N})
    &\defeq
       \sum_{\vb: \, \text{$\vx$ fixed}}
         Q
           \big(\vx 
           \big| 
           \vx_{-\infty}^{-N}
           \big.
           \big) \, 
         W(\vb, \vy | \vx, s_{-N}), \\
  (QW)(\vy|s_{-N})
    &\defeq
       \sumb
         \big(\vx 
           \big| 
           \vx_{-\infty}^{-N}
           \big.
           \big) \, 
         W(\vb, \vy | \vx, s_{-N}).
\end{align}




  


\begin{Definition}{Data-Controllable FSMCs}
  \label{def:controlable}

  If an indecomposable finite-state machine channel can be taken from any
  state into any other state by a finite number of channel inputs, which do
  not depend on the current state, the channel is called {\em controllable}.
  (Referring to~\cite[p.~111 and p.~527]{Gallager:68}, we note that there are
  also decomposable channels that could be called controllable and for which
  the unconstrained capacity is uniquely defined. However, in the following we
  will not consider such channels because we deal exclusively with
  indecomposable channels.)
\end{Definition}

Clearly, the partial response channel in
Ex.~\ref{ex:partial:response:channel:1} is data-controllable, whereas the
Gilbert-Elliott channel (cf.~\ref{example:gilbert:elliott:channel:1}) is
\emph{not} data-controllable.




\subsection{\textbf{General Channels with Memory}}
\label{sec:general:channels:memory:1}


In general, we will allow a the original channels to be more general than
indecomposable FSMCs, namely, we allow the state-space size to be infinite, as
long as the following requirement is satisfied: if the channel is fed with a
stationary and ergodic source then the input and output processes must be
jointly stationary and ergodic processes. In particular, we require that the
channels behave like indecomposable FSMCs, \ie, that the influence of the
initial state fades out with time for every possible channel input sequence.



\subsection{\textbf{Backward Channel Model}}
\label{sec:backward:channel:model:1}


Reversing the usual meaning of $\vX$ and $\vY$, i.e., looking at $\vX$ as
being the output of some channel which is fed by $\vY$ which in turn is
produced by some source, we arrive at the ``backward'' channel model in
Fig.~\ref{fig:source:channel:prob:models:1}(b). Note that the mutual
information $I(\vX;\vY)$ is a functional of the joint pmf of $\vX$ and $\vY$.
Therefore, if $\vX$ and $\vY$ have the same joint pmf in both the forward and
the backward channel setup then both channels will have the same information
rate. This can be achieved by setting the pmf of the ``output'' source to be
$R(\vy) \defeq (QW)(\vy)$ and the ``backward'' channel law to be $V(\vx|\vy) =
\frac{Q(\vx) W(\vy|\vx)}{(QW)(\vy)}$ because then $Q(\vx) W(\vy) = R(\vy)
V(\vx|\vy)$.


\subsection{\textbf{Forward Auxiliary Finite-State Machine Channels}}
\label{sec:forward:aux:finite:state:channel:models:1}


The information rate upper bounds in \secref{sec:information:rate:bound:1}
will be based on a forward auxiliary channel law. By a forward auxiliary
channel law we will simply mean a conditional pmf on $\vy$ given $\vx$. In
general, we will denote this conditional pmf by $\What(\vy|\vx)$ and it
fulfills the usual properties of a conditional pmf, i.e., $\What(\vy|\vx) \geq
0$ for all $\vx$ and all $\vy$, and $\sum_{\vy} \What(\vy|\vx) = 1$ for all
$\vx$.

In the following, we will focus on the case where the forward auxiliary
channel is a forward auxiliary finite-state machine channel (FA-FSMC).



\begin{Definition}{FA-FSMCs}
  \label{def:forward:aux:finite:state:channel:models:1}

  A time-independent and discrete-time FA-FSMC has an input process $\ldots,
  X_{-1}, X_0, X_1, \ldots$, an output process $\ldots, \hat
  Y_{-1}, Y_0, Y_1, \ldots$, and a state process $\ldots$,
  $\Shat_{-1}$, $\Shat_0$, $\Shat_1$, $\ldots$, where $X_{\ell} \in \hat
  \setX$, $Y_{\ell} \in \setY$, and $\Shat_{\ell} \in \setShat$ for
  all $\ell \in {\mathbb Z}$. We assume the sets $\setX$, $\setY$, and
  $\setShat$ to be finite.\footnote{Clearly, the finite-ness of $\setX$ and
    $\setY$ is induced by the finite-ness of $\setX$ and $\setY$.} Let us
  define the following finite windows of the FA-FSMC states and branches as:
  \begin{align}
    \vshat
      &\defeq
         {\vshat}_{-N+1}^{N},
    \quad\quad
    \vbhat
       \defeq
         {\vbhat}_{-N+1}^{N}.
  \end{align}
  The FA-FSMC conditional pmf decomposes as
  \begin{align}
    \What(\vshat, \vy | \vx, \shat_{-N})
      &= \prod_{\ell \in \sIN}
           \What(\shat_{\ell}, y_{\ell} | \shat_{\ell-1}, x_{\ell}) 
               \label{eq:aux:FSMC:decompose:2}
       = \left(
           \prod_{\ell \in \sIN}
             \What(\shat_{\ell} | \shat_{\ell-1}, x_{\ell})
         \right)
         \cdot
         \left(
           \prod_{\ell \in \sIN}
             \What(y_{\ell} |  \shat_{\ell-1}, x_{\ell}, \shat_{\ell})
         \right),
  \end{align}
  where $\What(\shat_{\ell} | \shat_{\ell-1}, x_{\ell})$ and $\What(y_{\ell} |
  \shat_{\ell-1}, x_{\ell}, \shat_{\ell})$ are referred to as the auxiliary
  FSMC state transition probability and channel law in each state transition,
  respectively and are independent of time index $\ell$. The input-output
  conditional pmf will then be\footnote{CCCCC Quickly talk about uniqueness of
    branches.}
  \begin{align}
    \What(\vy | \vx, \shat_{-N})
      &\defeq
         \sum_{\vshat}
           \What(\vshat, \vy | \vx, \shat_{-N}).
  \end{align}
\end{Definition}


It is useful to introduce the auxiliary FSMC branch random variable
$\Bhat_{\ell} \defeq (\Shat_{\ell-1}, X_{\ell}, \Shat_{\ell})$. The initial
state of a branch $\bhat_{\ell}$ at time index $\ell$ will then be denoted by
$\shat_{\ell-1}(\bhat_{\ell})$, the channel input symbol by $x(\bhat_{\ell})$,
and the final state by $\shat_{\ell}(\bhat_{\ell})$. In that sense, we will
often write $\What(y_{\ell} | \bhat_{\ell})$ instead of $\What(y_{\ell} |
\shat_{\ell-1}, x_{\ell}, \shat_{\ell})$, and $\What(\vbhat, \vy | \vx,
\shat_{-N})$ instead of $\What(\vshat, \vy | \vx, \shat_{-N})$ if $\vbhat =
(\vx, \vshat)$.


\begin{Remark}
  \label{remark:induced:pmfs:1}

  Of special interest is the case where $\vx$ is generated according to the
  standard source: the induced joint pmf of $\vx$, $\vshat$, and $\vy$ is then
  called $\Phat(\vx,\vshat,\vy)$ and equals $\Phat(\vx,\vshat,\vy) \defeq
  Q(\vx) \What(\vshat, \vy|\vx)$. In that sense,
  \begin{align}
    \Phat(\vbhat,\vy)
      &= \Phat(\vx,\vshat,\vy), \\
    \Phat(\vx, \vy | \shat_{-N})
      &\defeq
         \sum_{\vshat}
           \Phat(\vx,\vshat,\vy | \shat_{-N}), \\
    \Phat(\vy | \shat_{-N})
      &\defeq
         \sum_{\vx, \, \vshat}
           \Phat(\vx, \vshat, \vy | \shat_{-N})
       = \sum_{\vx}
           \Phat(\vx, \vy | \shat_{-N})
       = (Q\What)(\vy | \shat_{-N}), \\
    \Phat(\vbhat | \vy, \shat_{-N})
      &\defeq
         \frac{\Phat(\vbhat, \vy | \shat_{-N})}
              {\Phat(\vy | \shat_{-N})}, \\
    \Phat(\vbhat | \vx, \vy, \shat_{-N})
      &\defeq
         \frac{\Phat(\vbhat, \vy | \shat_{-N})}
              {\sum\limits_{\vbhat': \, 
                           \text{$\vbhat'$ is compatible with $\vx$}}
                 \Phat(\vbhat', \vy | \shat_{-N})},
  \end{align}
  where in the last expression we assume that $\vx$ is compatible with
  $\vbhat$.
\end{Remark}









\subsection{\textbf{Backward Auxiliary Finite-State Machine Channels}}
\label{sec:backward:aux:finite:state:channel:models:1}


The information rate lower bounds in \secref{sec:information:rate:bound:1}
will be based on a backward auxiliary channel law. By a backward auxiliary
channel law we will simply mean a conditional pmf on $\vx$ given $\vy$. In
general, we will denote this conditional pmf by $\Vhat(\vx|\vy)$ and it
fulfills the usual properties of a conditional pmf, i.e., $\What(\vx|\vy) \geq
0$ for all $\vx$ and all $\vy$, and $\sum_{\vx} \What(\vx|\vy) = 1$ for all
$\vy$.

In the following, we will focus on the case where the forward auxiliary
channel is a backward auxiliary finite-state machine channel (BA-FSMC).



\begin{Definition}{BA-FSMCs}
  \label{def:backward:aux:finite:state:channel:models:1}

  A time-independent and discrete-time BA-FSMC has an input process $\ldots,
  X_{-1}, X_0, X_1, \ldots$, an output process $\ldots, \hat
  Y_{-1}, Y_0, Y_1, \ldots$, and a state process $\ldots$,
  $\Shat_{-1}$, $\Shat_0$, $\Shat_1$, $\ldots$, where $X_{\ell} \in \hat
  \setX$, $Y_{\ell} \in \setY$, and $\Shat_{\ell} \in \setShat$ for
  all $\ell \in {\mathbb Z}$. We assume the sets $\setX$, $\setY$, and
  $\setShat$ to be finite.\footnote{Clearly, the finite-ness of $\setX$ and
    $\setY$ is induced by the finite-ness of $\setX$ and $\setY$.} Let us
  define the following finite windows of the FA-FSMC states and branches as:
  \begin{align}
    \vshat
      &\defeq
         {\vshat}_{-N+1}^{N},
    \quad\quad
    \vbhat
       \defeq
         {\vbhat}_{-N+1}^{N}.
  \end{align}
  The BA-FSMC conditional pmf is defined to be
  \begin{align}
    \Vhat(\vshat, \vx | \vy, s_{-N})
      &\defeq
         \frac{\vhat(\vshat, \vx, \vy | s_{-N})}
              {\sum\limits_{\vshat', \vx'}
                 \vhat(\vshat', \vx', \vy | s_{-N})}
         \label{eq:backward:auxiliary:channel:law:1}
  \end{align}
  with
  \begin{align}
    \vhat(\vshat, \vx, \vy | s_{-N})
      &\defeq
         Q(\vx)
         \cdot
         \prod_{\ell \in \sIN}
           \vhat
             \left(
               \shat_{\ell-1}, x_{\ell}, s_{\ell}, \vy_{\ell-D_1}^{\ell+D_2}
             \right).
         \label{eq:backward:auxiliary:channel:law:1:part:2}
  \end{align}
  Here, $D_1$ and $D_2$ are some arbitrary non-negative integers and
  $\vhat(\vshat_{\ell-1}, x_{\ell}, s_{\ell}, \vy_{\ell-D_1}^{\ell+D_2})$ is a
  non-negative function of $\shat_{\ell-1}$, $x_{\ell}$, $\shat_{\ell}$, and
  $\vy_{\ell-D_1}^{\ell+D_2}$ and $s_{-N}$; the latter requirement is
  sufficient for $\Vhat(\vshat, \vx | \vy, s_{-N})$ to represent a conditional
  pmf of $\vshat$ and $\vx$ given $\vy$ and $s_{-N}$.\footnote{The letter
    $\vhat$ was chosen to show the closeness of the $\vhat$ function to the
    $\Vhat$ function, yet to remind the reader that it is not properly
    normalized to be a conditional pmf of $\vshat$ and $\vx$ given $\vy$ and
    $s_{-N}$.}  The backward input-output conditional pmf will then
  be\footnote{CCCCC Quickly talk about uniqueness of branches.}
  \begin{align}
    \Vhat(\vx | \vy, \shat_{-N}) &\defeq \sum_{\vshat} \Vhat(\vshat, \vx |
    \vy, \shat_{-N}).
  \end{align}
\end{Definition}


In the following, we will also use
\begin{align*}
  \Vhat(\vshat | \vx, \vy, \shat_{-N})
    &\defeq
       \frac{\Vhat(\vshat, \vx | \vy, \shat_{-N})}
            {\sum_{\vshat'}
               \Vhat(\vshat', \vx | \vy, \shat_{-N})}
     = \frac{\vhat(\vshat, \vx, \vy | \shat_{-N})}
            {\sum_{\vshat'}
               \vhat(\vshat', \vx, \vy | \shat_{-N})}.
\end{align*}
It is useful to introduce the auxiliary FSMC branch random variable
$\Bhat_{\ell} \defeq (\Shat_{\ell-1}, X_{\ell}, \Shat_{\ell})$. The initial
state of a branch $\bhat_{\ell}$ at time index $\ell$ will then be denoted by
$\shat_{\ell-1}(\bhat_{\ell})$, the channel input symbol by $x(\bhat_{\ell})$,
and the final state by $\shat_{\ell}(\bhat_{\ell})$. In that sense, we will
often write $\vhat(\bhat_{\ell}, \vy_{\ell-D_1}^{\ell+D_2})$ instead of
$\vhat(\vshat_{\ell-1}, x_{\ell}, s_{\ell}, \vy_{\ell-D_1}^{\ell+D_2})$,
$\Vhat(\vbhat | \vy, \shat_{-N})$ instead of $\What(\vshat, \vx | \vy,
\shat_{-N})$ if $\vbhat = (\vx, \vshat)$, and $\Vhat(\vbhat | \vx, \vy,
\shat_{-N})$ instead of $\Vhat(\vshat | \vx, \vy, \shat_{-N})$ if $\vbhat =
(\vx, \vshat)$.


\subsection{\textbf{Remarks}}


Let us briefly point out some notational differences with the notation used in
the paper on the generalized Blahut-Arimoto
Algoritm~\cite{Vontobel:Kavcic:Arnold:Loeliger:04:1:subm}. Similarly to that
paper, we are using $\vx$ and to denote the source output / channel input
sequence and $\vy$ to denote the channel output sequence.  However, in the
current paper $\vs$ and $\vb$ denote the state and branch sequence,
respectively, in the trellis representation of the \emph{channel}, whereas
in~\cite{Vontobel:Kavcic:Arnold:Loeliger:04:1:subm}, $\vs$ and $\vb$ were used
to denote the state and branch sequence, respectively, in the trellis
representation of the \emph{source}. Finally, note that in both papers the
time indexing of the components of the input, output, state, and branch
sequences are done in the same manner, however, $\vs$ is defined to be
$\vs_{-N+1}^{N}$ and not $\vs_{-N}^{N}$.


We have already mentioned that we will be mainly interested in the limit $N
\to \infty$. Because our setup is such that the limits of the expressions of
interest do not depend on the past $\vx_{-\infty}^{-N}$ and the initial states
$s_{-N}$ and $\shat_{-N}$ (this can be justified using results like
in~\cite{LeGland:Mevel:00:2}), in the following we will assume that
$\vx_{-\infty}^{-N}$, $s_{-N}$, and $\shat_{-N}$ are fixed to some suitable
and mutually compatible values. In order to simplify the notation in all the
upcoming formulas, we will omit the explicit conditioning on
$\vx_{-\infty}^{-N}$, $s_{-N}$, and $\shat_{-N}$, however, it should be kept
in mind that such a conditioning is still present.



CCCCC If not already done, somewhere we have to introduce the generic
$\shatL$, $\shat$, $x$.

